Why Quantization Improves Generalization: NTK of Binary Weight Neural Networks

Quantized neural networks have drawn a lot of attention as they reduce the space and computational complexity during the inference. Moreover, there has been folklore that quantization acts as an implicit regularizer and thus can improve the generalizability of neural networks, yet no existing work formalizes this interesting folklore. In this paper, we take the binary weights in a neural network as random variables under stochastic rounding, and study the distribution propagation over different layers in the neural network. We propose a quasi neural network to approximate the distribution propagation, which is a neural network with continuous parameters and smooth activation function. We derive the neural tangent kernel (NTK) for this quasi neural network, and show that the eigenvalue of NTK decays at approximately exponential rate, which is comparable to that of Gaussian kernel with randomized scale. This in turn indicates that the Reproducing Kernel Hilbert Space (RKHS) of a binary weight neural network covers a strict subset of functions compared with the one with real value weights. We use experiments to verify that the quasi neural network we proposed can well approximate binary weight neural network. Furthermore, binary weight neural network gives a lower generalization gap compared with real value weight neural network, which is similar to the difference between Gaussian kernel and Laplace kernel.

==> response.tex <==
\section{Response to reviewers}

% I think for each reviewer, you can firstly thank their efforts and suggestions. And if they acknowledged any advantage of your paper, you may point them out in some way like "We appreciate that reviewers found our system ... and acknowledged the .... We value the critiques and suggestions as they help us better communicate our insights ...". This will restate the pros to the reviewers and should be helpful for your rebuttal.

% For modifications you want to make to the paper, you may briefly write them in the rebuttal, and point out which section they will be added to. 

\subsection{Reviewer 1 (ALLp)}
We would like to thank the reviewer for your feedback, and for acknowledging the two steps we used in the proof. However, recent studies show that step 1 isn't as straightforward as it looks like.
However, we respectively disagree with the reviewer's assessment that step 1 is straightforward and step 2 is invalid.
%However, we disagree on the reviewer's comment that step 1 is straightforward. 
Firstly, as has been shown by various numerical results, although a neural network can approximate a wide class of functions, the training dynamics and early stopping limits the the function after training to a smaller class (aka, the RKHS of the kernel). Studying the function class that can be reached by training is the main motivation of this paper. Secondly, although it is true that a finite width neural network has larger capacity that the binary weight counterpart, this is not necessarily true for infinite wide ones. A naive idea is to use repeat a neuron several times in a binary weight neural network to approximate one with real weights. For step 2, the relationship between model capacity and generalization has been proved in many different work from different perspectives, eg. ``Rademacher and Gaussian complexities: Risk bounds and structural results.'', Journal of Machine Learning Research 3.Nov (2002): 463-482., Barbiero, Pietro, Giovanni Squillero, and Alberto Tonda. ``Modeling generalization in machine learning: A methodological and computational study.''. Your comment that ``smaller network capacity does not necessary imply better generalization'' is exactly right and it is the very reason we consider using the NTK to study the behaviors of quantized NNs. To our understanding, NTK (partly) explains the generalization of neural network by studying the capacity of a neural network from its training dynamics.


\subsection{Reviewer 2 (33GU)}
We would like to thank the reviewer for reading this paper and providing valuable feedback. Below is the response to the detailed comments.

1. Note that the linear layer before $x_1$ is not quantized and not trained, under the condition of real-valued model parameters $\theta_0, \theta_1, \theta_2$, $x_1$ is fixed.

We appreciate the reviewer's follow-up comment. 
Lemma 1 contains two parts: the first part is to compute the mean and variance of $y_{1, j}$ conditioned on $\Theta$, which holds true regardless of the value or initialization method of $\Theta$. The second part states that if one sample a series of parameters $\Theta^{(d)}$ with width of neural network $d$ growing to infinity, and for each $\Theta^{(d)}$ one can compute (the distribution of) $y_{1, j}$ denoted as $y_{1, j}^{(d)}$, then with high probability,  $y_{1, j}^{(d)}$ converges to Gaussian distribution. We are sorry for the confusion and hope this clarifies the statement.

Lazy training has been widely observed and in overparameterized neural networks and proven in several different papers, eg. Allen-Zhu, Zeyuan, Yuanzhi Li, and Zhao Song. " A convergence theory for deep learning via over-parameterization." International Conference on Machine Learning. PMLR, 2019. We recognize that this property hasn't been proven for binary weight neural network to our best knowledge. The original NTK paper made the assumption that the total updates $\int_0^T \|d_t\|_{p^{in}}dt$ stays stochastically bounded as width grow to infinity. We wonder whether it will be satisfying if we make similar assumption in this paper and prove the convergence of kernel from this point. We appreciate your feedback.



2. There's some editing errors in the original version of Thm 3. We're sorry for the confusion. The improved version is attached below: %\textcolor{red}{[Say which theorem this replaces...]}

Under random initialization of $\Theta$, the mean of the output of the first layer conditioned on $\Theta$, aka $\varsigma_{1, j}$, aka $\nu_{1, j}$ converges to Gaussian random variables which are independent from each other, and variance of output of the first linear layer conditioned on $\Theta$, aka $\varsigma_{1, j}$ converges almost surely to 
\begin{equation*}
    \tilde\varsigma_1^2 = \frac{c}{d_1}(1-\E[\theta_{1,ij}^2])\E[{x_{1, i}}^2]
    = \frac{c}{d}(1-\Var[\theta]).
\end{equation*}

3. The expectations in thm 4 \& 5 are taken under the randomness of stochastic rounding, aka. $w_1$, and conditioned on initialization.

4. In lazy training regime, model parameters stay close to their initialization point throughout training process, which indicates that theorem 4 and 5 are reasonable approximation throughout training process as long as the model stays in lazy training regime.

\subsection{Reviewer 4 (DxRf)}
We would like to thank the reviewer for reading this paper and providing valuable feedback. Below is the response to the detailed comments.

1. We will modify the title of section 5 to ``capacity of Binary Weight Neural Network'' and add more discussion to draw the connection between model capacity and NTK, eg. the effective capacity of a neural network is equivalent to the RKHS of its NTK. 

2. 3. We will add more detail about the experiment results, including generalization gap,  and modify these parts accordingly in the later version.


\subsection{Reviewer 4 (on8h)}
We would like to thank the reviewer for reading this paper and providing valuable feedback. Below is the response to the detailed comments.

1. The motivation of studying a partly quantized neural network is two-folded. 1) This makes the discussing simpler, and eliminates the need to introduce more symbols. We hope that once a reader gets the idea of partly quantized neural network, one can easily expand the result to fully quantized neural network, which is the same as partly quantized ones. 2) In empirical work researchers often leave the last layer (sometimes together with the first layer) not quantized to improve empirical performance, eg. Zhou, Shuchang, et al. ``Dorefa-net: Training low bitwidth convolutional neural networks with low bitwidth gradients.'' arXiv preprint arXiv:1606.06160 (2016), Rastegari, Mohammad, et al. ``Xnor-net: Imagenet classification using binary convolutional neural networks.'' European conference on computer vision. Springer, Cham, 2016. %(\textcolor{red}{add a citation here?})
We hope this helps our result to cover these cases more easily.

2. The first layer refers to the linear layer between $x_1$ and $y_1$ (or $\nu_1$), and the second layer refers to the linear layer between $x_2$ (or $\mu_2$) to $y$ (or $\bar y$). $w_{2, j}$ is a typo for $\theta_{2, j}$. Line 181 should look like ``then the output $x_{2,j}$ has mean $\mu_{2,i}$ and variance $\sigma_{2,i}^2$ conditioned on $\Theta$ ''. We appreciate the review for pointing this out and apologize for the editing error. 

3. We will modify the figure in the next version. Nodes will be dedicated for variables and functions will be represented by arrows.

4. The connection between model complexity and generalization has been proven both empirically and theoretically in many works, e.g. Bartlett, Peter L., and Shahar Mendelson. ``Rademacher and Gaussian complexities: Risk bounds and structural results.'', Journal of Machine Learning Research 3.Nov (2002): 463-482., Barbiero, Pietro, Giovanni Squillero, and Alberto Tonda. ``Modeling generalization in machine learning: A methodological and computational study.'' arXiv preprint arXiv:2006.15680 (2020). When people compare the performance of BWNN and NN, in most of the cases only testing error is compared, and potentially training error might be compensated by smaller generalization gap. 

5. 6. Thanks for the advise. We will add more data to the later version, including the percentage of datasets that BWNN do better. We wonder what does it mean by error? To our understanding, error = 1 - accuracy.

7. Thanks for the advise on application. Theoretically BWNN-NTK can be used in the same way as NTK, while a potential barrier is that we don't have an efficient way to compute it analytically.
